A Unified Model for High-Resolution ODEs: New Insights on Accelerated Methods

Recent work on high-resolution ordinary differential equations (HR-ODEs) captures fine nuances among different momentum-based optimization methods, leading to accurate theoretical insights. However, these HR-ODEs often appear disconnected, each targeting a specific algorithm and derived with different assumptions and techniques. We present a unifying framework by showing that these diverse HR-ODEs emerge as special cases of a general HR-ODE derived using the Forced Euler-Lagrange equation. Discretizing this model recovers a wide range of optimization algorithms through different parameter choices. Using integral quadratic constraints, we also introduce a general Lyapunov function to analyze the convergence of the proposed HR-ODE and its discretizations, achieving significant improvements across various cases, including new guarantees for the triple momentum method$'$s HR-ODE and the quasi-hyperbolic momentum method, as well as faster gradient norm minimization rates for Nesterov$'$s accelerated gradient algorithm, among other advances.

==> Fig3a.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{mycolor2}{rgb}{0.85000,0.32500,0.09800}%
\definecolor{mycolor3}{rgb}{0.92900,0.69400,0.12500}%
%
\begin{tikzpicture}

\begin{groupplot}[
        group style={group name=fig3,group size=2 by 1, horizontal sep=2cm
        },   
        width=0.465\textwidth, 
        height=0.395\textwidth,        
        %xlabel={Epoch},
        % legend style={at={(0.5,1.3)}, anchor=north,legend columns=3},        
        % legend cell align={center},        
        grid=both, grid style={gray!30},        
        tick label style={font=\footnotesize}, 
        ]
    
    % First subplot: training error
\nextgroupplot[
    ymin=1e-15, ymax=1e2,
    xmin=1e0, xmax=1e2,  
    ylabel={\(f(x_k)-f(x^*)\)}, 
    xlabel={Iteration},
    %ytick distance=2,
    line width=0.1pt,
    xtick align=outside,
    ytick align=outside,
    %xmode=log,
    ymode=log,
    ]
\addplot [color=mycolor1, line width=2.5pt]
  table[row sep=crcr]{%
1	210.095562436466\\
2	174.267152871458\\
3	126.941603897643\\
4	71.7324572481976\\
5	11.9346632646616\\
6	0.643617944910188\\
7	2.26593197483689\\
8	4.16391748760623\\
9	5.9993287826018\\
10	7.58574489921796\\
11	8.83676333006101\\
12	9.72960808869808\\
13	10.2799278421884\\
14	10.5246609906501\\
15	10.510662481992\\
16	10.2874003299502\\
17	9.90248779423209\\
18	9.39915784486114\\
19	8.81503875060043\\
20	8.18177538799921\\
21	7.52517685848794\\
22	6.86566987281051\\
23	6.21890866856726\\
24	5.59644316304305\\
25	5.00638301095583\\
26	4.45402027476312\\
27	3.94239053244771\\
28	3.47276367498876\\
29	3.04506302830117\\
30	2.658215978608\\
31	2.31044186443264\\
32	1.99948415734652\\
33	1.72279434185219\\
34	1.47767474501624\\
35	1.26138708629761\\
36	1.07123287816467\\
37	0.904611123522105\\
38	0.759058109831239\\
39	0.632273548677836\\
40	0.522136878513104\\
41	0.42671721733901\\
42	0.344280139797628\\
43	0.273294005761856\\
44	0.212437754916451\\
45	0.160610585467698\\
46	0.116941312205603\\
47	0.0807908716467565\\
48	0.0517349786586425\\
49	0.029506287951665\\
50	0.0138718807635229\\
51	0.00443581272405988\\
52	0.000405747876149803\\
53	0.000443905761938007\\
54	0.00276726365101393\\
55	0.00555588963231965\\
56	0.00747780504603743\\
57	0.00799103331403131\\
58	0.00725272359162116\\
59	0.00577645790523598\\
60	0.00409747662463517\\
61	0.00259112757962357\\
62	0.00143878391923521\\
63	0.000672168914798099\\
64	0.000236521269773193\\
65	4.27581116657916e-05\\
66	8.05116577823339e-07\\
67	3.6506961688304e-05\\
68	9.72987949741377e-05\\
69	0.000151359939729617\\
70	0.000183643291051389\\
71	0.000190925578930329\\
72	0.000177101601337187\\
73	0.000149332143164621\\
74	0.000115268107690608\\
75	8.13367394512654e-05\\
76	5.1937813102948e-05\\
77	2.9327401049134e-05\\
78	1.39465069800282e-05\\
79	4.96931433602299e-06\\
80	8.89700076167621e-07\\
81	2.27064870794713e-08\\
82	8.57408629567624e-07\\
83	2.24858649885973e-06\\
84	3.47024628627457e-06\\
85	4.17246849349073e-06\\
86	4.28649264580527e-06\\
87	3.91603779278937e-06\\
88	3.24087839306819e-06\\
89	2.4460937029791e-06\\
90	1.68006966480561e-06\\
91	1.03750882229914e-06\\
92	5.60383039249768e-07\\
93	2.4919075217178e-07\\
94	7.80374178055432e-08\\
95	8.99711341539877e-09\\
96	3.22838580868456e-09\\
97	2.7985179507084e-08\\
98	5.98074949564875e-08\\
99	8.4795231919399e-08\\
100	9.63718636837196e-08\\
};\label{figNag3}
%\addlegendentry{Nesterov}

\addplot [color=mycolor2, dashdotted, line width=2.5pt]
  table[row sep=crcr]{%
1	210.095562436466\\
2	192.310448333424\\
3	155.211091896182\\
4	104.276550830535\\
5	44.2253111777479\\
6	0.0336653136927416\\
7	1.00105716395343\\
8	2.42635112215863\\
9	3.882010749747\\
10	5.1545785197657\\
11	6.14707568252227\\
12	6.83369658335104\\
13	7.2295977202392\\
14	7.37118767254353\\
15	7.30364153914042\\
16	7.07331816083508\\
17	6.72344776634928\\
18	6.29195296585163\\
19	5.81061980792334\\
20	5.30508665891702\\
21	4.79529542149194\\
22	4.29617292742777\\
23	3.81839543247452\\
24	3.3691470687553\\
25	2.95282187982538\\
26	2.57164444266347\\
27	2.22620020156702\\
28	1.91587644259716\\
29	1.63922040301953\\
30	1.39422379665988\\
31	1.1785440594262\\
32	0.989672584891191\\
33	0.825059618297787\\
34	0.682204648895392\\
35	0.558720308357574\\
36	0.452377054995153\\
37	0.361135269680054\\
38	0.283170614664236\\
39	0.216897233958728\\
40	0.160991026831913\\
41	0.11441096537433\\
42	0.0764091029924071\\
43	0.0465085702070367\\
44	0.0244152900393521\\
45	0.00982466940047605\\
46	0.00211771322490945\\
47	4.46516842905198e-05\\
48	0.00163448391721482\\
49	0.00456445500960301\\
50	0.00689661155254484\\
51	0.00767895504621979\\
52	0.00697271818035508\\
53	0.00539825978246053\\
54	0.00362797620762034\\
55	0.00211080066519534\\
56	0.00103194129288026\\
57	0.000388880948158615\\
58	8.55171654220166e-05\\
59	1.70082730363563e-06\\
60	3.17894311252231e-05\\
61	9.97576802620748e-05\\
62	0.000160298912705109\\
63	0.000193158037306879\\
64	0.000195274474078799\\
65	0.000173270969659606\\
66	0.000137486022265543\\
67	9.79323553117473e-05\\
68	6.20880795473289e-05\\
69	3.416805249154e-05\\
70	1.54110138688157e-05\\
71	4.91377969649709e-06\\
72	6.17030762595228e-07\\
73	1.66639491872012e-07\\
74	1.50662734027529e-06\\
75	3.17504522337475e-06\\
76	4.353092092374e-06\\
77	4.7550876305924e-06\\
78	4.44887926051574e-06\\
79	3.67596705450057e-06\\
80	2.7119724739233e-06\\
81	1.78161990366243e-06\\
82	1.02377429681e-06\\
83	4.92502746057832e-07\\
84	1.77992959621287e-07\\
85	3.37122864624284e-08\\
86	7.55407764119198e-10\\
87	2.4952412081003e-08\\
88	6.59030695293605e-08\\
89	9.9306634082641e-08\\
90	1.14886703983519e-07\\
91	1.12218752651438e-07\\
92	9.62550244787419e-08\\
93	7.36478176777133e-08\\
94	5.0329638817681e-08\\
95	3.03377770960456e-08\\
96	1.56025845854391e-08\\
97	6.32636423802957e-09\\
98	1.60914667701739e-09\\
99	7.06291414243054e-11\\
100	1.2720110242892e-09\\
};\label{figGMSIE12}
%\addlegendentry{$\text{GM-SIE}^\text{1}$}

\addplot [color=mycolor3, dashed, line width=2.5pt]
  table[row sep=crcr]{%
1	210.095562436466\\
2	174.267152871458\\
3	127.980266203922\\
4	74.3545003883637\\
5	16.1535214325929\\
6	0.490294572156493\\
7	1.97157294565933\\
8	3.79345197592255\\
9	5.63156041503103\\
10	7.2917008807982\\
11	8.66997933130001\\
12	9.72352197571708\\
13	10.4491921897046\\
14	10.8683429999437\\
15	11.0160876184419\\
16	10.933921665481\\
17	10.664805628456\\
18	10.250030469102\\
19	9.72735573219248\\
20	9.13003813616659\\
21	8.48646752131536\\
22	7.82020263456053\\
23	7.1502566594202\\
24	6.49152571000438\\
25	5.85528590043916\\
26	5.2497085953561\\
27	4.68036101815712\\
28	4.15067208398013\\
29	3.66235233274037\\
30	3.21576309215645\\
31	2.81023421551131\\
32	2.44433246067944\\
33	2.11608422140244\\
34	1.82315720303525\\
35	1.56300598904181\\
36	1.3329864485938\\
37	1.13044372429899\\
38	0.952778218007156\\
39	0.797493648774435\\
40	0.662230962482316\\
41	0.544791677353198\\
42	0.443154160715038\\
43	0.355486282037072\\
44	0.280157700148391\\
45	0.215754410385839\\
46	0.161096629813816\\
47	0.115257939690241\\
48	0.0775778454671363\\
49	0.0476505473511532\\
50	0.0252603944573988\\
51	0.01022637793234\\
52	0.0021351022441711\\
53	1.59277894344889e-05\\
54	0.00214247143292806\\
55	0.00621504527362621\\
56	0.00999048374764144\\
57	0.0120156071220268\\
58	0.011945628657265\\
59	0.0102845764447449\\
60	0.00785469186159757\\
61	0.00537403842419354\\
62	0.00328237254977562\\
63	0.00175188051348202\\
64	0.000772873713916128\\
65	0.000242467256778151\\
66	2.8731768621254e-05\\
67	7.99936665890622e-06\\
68	8.19543216838692e-05\\
69	0.000182048957193759\\
70	0.000267049584158463\\
71	0.000317514579977196\\
72	0.000329462344018094\\
73	0.000308462357188954\\
74	0.000264750865485469\\
75	0.000209595266945695\\
76	0.000152906130338137\\
77	0.000101960067661833\\
78	6.1017039011263e-05\\
79	3.15770829886763e-05\\
80	1.30177536180609e-05\\
81	3.3802176547526e-06\\
82	1.22101013133591e-07\\
83	7.1844438170876e-07\\
84	3.05644094461544e-06\\
85	5.62403982584669e-06\\
86	7.52986120586274e-06\\
87	8.41006355375984e-06\\
88	8.27925120916451e-06\\
89	7.37246363996524e-06\\
90	6.00976062450909e-06\\
91	4.49902365992627e-06\\
92	3.07966765072942e-06\\
93	1.90144623984922e-06\\
94	1.02840295862494e-06\\
95	4.57349076360414e-07\\
96	1.41793459557116e-07\\
97	1.48363061835965e-08\\
98	7.27312540749203e-09\\
99	5.948165679448e-08\\
100	1.83301257006274e-07\\
};\label{figshiSIE2}
%\addlegendentry{Shi-SIE}

\nextgroupplot[
        ymin=1e-10, ymax=1e5,   
        xmin=0, xmax=1e2,  
        ylabel={\(f(x_k)-f(x^*)\)},    
        %ytick distance=0.1,
        xlabel={Iteration},
        line width=0.7pt,
        xtick align=outside,
        ytick align=outside,
        ymode = log,
        %xmode = log,
        ]


\addplot [color=mycolor1, line width=2.5pt]
  table[row sep=crcr]{%
1	210.095562436466\\
2	174.267152871458\\
3	126.941603897643\\
4	71.7324572481976\\
5	11.9346632646616\\
6	0.643617944910188\\
7	2.26593197483689\\
8	4.16391748760623\\
9	5.9993287826018\\
10	7.58574489921796\\
11	8.83676333006101\\
12	9.72960808869808\\
13	10.2799278421884\\
14	10.5246609906501\\
15	10.510662481992\\
16	10.2874003299502\\
17	9.90248779423209\\
18	9.39915784486114\\
19	8.81503875060043\\
20	8.18177538799921\\
21	7.52517685848794\\
22	6.86566987281051\\
23	6.21890866856726\\
24	5.59644316304305\\
25	5.00638301095583\\
26	4.45402027476312\\
27	3.94239053244771\\
28	3.47276367498876\\
29	3.04506302830117\\
30	2.658215978608\\
31	2.31044186443264\\
32	1.99948415734652\\
33	1.72279434185219\\
34	1.47767474501624\\
35	1.26138708629761\\
36	1.07123287816467\\
37	0.904611123522105\\
38	0.759058109831239\\
39	0.632273548677836\\
40	0.522136878513104\\
41	0.42671721733901\\
42	0.344280139797628\\
43	0.273294005761856\\
44	0.212437754916451\\
45	0.160610585467698\\
46	0.116941312205603\\
47	0.0807908716467565\\
48	0.0517349786586425\\
49	0.029506287951665\\
50	0.0138718807635229\\
51	0.00443581272405988\\
52	0.000405747876149803\\
53	0.000443905761938007\\
54	0.00276726365101393\\
55	0.00555588963231965\\
56	0.00747780504603743\\
57	0.00799103331403131\\
58	0.00725272359162116\\
59	0.00577645790523598\\
60	0.00409747662463517\\
61	0.00259112757962357\\
62	0.00143878391923521\\
63	0.000672168914798099\\
64	0.000236521269773193\\
65	4.27581116657916e-05\\
66	8.05116577823339e-07\\
67	3.6506961688304e-05\\
68	9.72987949741377e-05\\
69	0.000151359939729617\\
70	0.000183643291051389\\
71	0.000190925578930329\\
72	0.000177101601337187\\
73	0.000149332143164621\\
74	0.000115268107690608\\
75	8.13367394512654e-05\\
76	5.1937813102948e-05\\
77	2.9327401049134e-05\\
78	1.39465069800282e-05\\
79	4.96931433602299e-06\\
80	8.89700076167621e-07\\
81	2.27064870794713e-08\\
82	8.57408629567624e-07\\
83	2.24858649885973e-06\\
84	3.47024628627457e-06\\
85	4.17246849349073e-06\\
86	4.28649264580527e-06\\
87	3.91603779278937e-06\\
88	3.24087839306819e-06\\
89	2.4460937029791e-06\\
90	1.68006966480561e-06\\
91	1.03750882229914e-06\\
92	5.60383039249768e-07\\
93	2.4919075217178e-07\\
94	7.80374178055432e-08\\
95	8.99711341539877e-09\\
96	3.22838580868456e-09\\
97	2.7985179507084e-08\\
98	5.98074949564875e-08\\
99	8.4795231919399e-08\\
100	9.63718636837196e-08\\
};\label{figNag4}
%\addlegendentry{Nesterov}

\addplot [color=mycolor2, dashed, line width=2.5pt]
  table[row sep=crcr]{%
1	210.095562436466\\
2	192.310448333424\\
3	155.211091896182\\
4	104.276550830535\\
5	44.2253111777479\\
6	0.0336653136927416\\
7	1.00105716395343\\
8	2.42635112215863\\
9	3.882010749747\\
10	5.1545785197657\\
11	6.14707568252227\\
12	6.83369658335104\\
13	7.2295977202392\\
14	7.37118767254353\\
15	7.30364153914042\\
16	7.07331816083508\\
17	6.72344776634928\\
18	6.29195296585163\\
19	5.81061980792334\\
20	5.30508665891702\\
21	4.79529542149194\\
22	4.29617292742777\\
23	3.81839543247452\\
24	3.3691470687553\\
25	2.95282187982538\\
26	2.57164444266347\\
27	2.22620020156702\\
28	1.91587644259716\\
29	1.63922040301953\\
30	1.39422379665988\\
31	1.1785440594262\\
32	0.989672584891191\\
33	0.825059618297787\\
34	0.682204648895392\\
35	0.558720308357574\\
36	0.452377054995153\\
37	0.361135269680054\\
38	0.283170614664236\\
39	0.216897233958728\\
40	0.160991026831913\\
41	0.11441096537433\\
42	0.0764091029924071\\
43	0.0465085702070367\\
44	0.0244152900393521\\
45	0.00982466940047605\\
46	0.00211771322490945\\
47	4.46516842905198e-05\\
48	0.00163448391721482\\
49	0.00456445500960301\\
50	0.00689661155254484\\
51	0.00767895504621979\\
52	0.00697271818035508\\
53	0.00539825978246053\\
54	0.00362797620762034\\
55	0.00211080066519534\\
56	0.00103194129288026\\
57	0.000388880948158615\\
58	8.55171654220166e-05\\
59	1.70082730363563e-06\\
60	3.17894311252231e-05\\
61	9.97576802620748e-05\\
62	0.000160298912705109\\
63	0.000193158037306879\\
64	0.000195274474078799\\
65	0.000173270969659606\\
66	0.000137486022265543\\
67	9.79323553117473e-05\\
68	6.20880795473289e-05\\
69	3.416805249154e-05\\
70	1.54110138688157e-05\\
71	4.91377969649709e-06\\
72	6.17030762595228e-07\\
73	1.66639491872012e-07\\
74	1.50662734027529e-06\\
75	3.17504522337475e-06\\
76	4.353092092374e-06\\
77	4.7550876305924e-06\\
78	4.44887926051574e-06\\
79	3.67596705450057e-06\\
80	2.7119724739233e-06\\
81	1.78161990366243e-06\\
82	1.02377429681e-06\\
83	4.92502746057832e-07\\
84	1.77992959621287e-07\\
85	3.37122864624284e-08\\
86	7.55407764119198e-10\\
87	2.4952412081003e-08\\
88	6.59030695293605e-08\\
89	9.9306634082641e-08\\
90	1.14886703983519e-07\\
91	1.12218752651438e-07\\
92	9.62550244787419e-08\\
93	7.36478176777133e-08\\
94	5.0329638817681e-08\\
95	3.03377770960456e-08\\
96	1.56025845854391e-08\\
97	6.32636423802957e-09\\
98	1.60914667701739e-09\\
99	7.06291414243054e-11\\
100	1.2720110242892e-09\\
};\label{figGMSIE1}
%\addlegendentry{$\text{GM-SIE}^\text{1}$}

\addplot [color=mycolor3, dotted, line width=2.5pt]
  table[row sep=crcr]{%
1	210.432534638163\\
2	192.551006016613\\
3	159.207462826889\\
4	114.698015876021\\
5	62.6695695791468\\
6	7.2397078152237\\
7	0.563326298300102\\
8	1.8534392147372\\
9	3.28768932347961\\
10	4.61622093229191\\
11	5.716232576669\\
12	6.54272539270462\\
13	7.09614808552883\\
14	7.40150989109017\\
15	7.49521875538816\\
16	7.41706559473942\\
17	7.20558829196232\\
18	6.89561468919847\\
19	6.51717570911527\\
20	6.0952498363338\\
21	5.64998521514121\\
22	5.19717142628723\\
23	4.74881777325988\\
24	4.31375138098826\\
25	3.8981854934072\\
26	3.50623225154009\\
27	3.14034923937474\\
28	2.80171816566059\\
29	2.49055923831591\\
30	2.20638746754354\\
31	1.94821823691032\\
32	1.71472963089259\\
33	1.50438861226963\\
34	1.31554746817818\\
35	1.14651615725251\\
36	0.995615394962181\\
37	0.86121457016122\\
38	0.741757924617854\\
39	0.635781860705137\\
40	0.54192576725371\\
41	0.458938354037583\\
42	0.385681134873781\\
43	0.321130361961393\\
44	0.264378345780283\\
45	0.214634642870394\\
46	0.171226994538578\\
47	0.133601080218179\\
48	0.101317051566404\\
49	0.0740394759994315\\
50	0.0515160626165021\\
51	0.0335402589327239\\
52	0.0198951423465242\\
53	0.0102829394683012\\
54	0.00425638541055817\\
55	0.00118065608456311\\
56	0.000257122905792218\\
57	0.000621235533577874\\
58	0.00148812534624609\\
59	0.00228524329576898\\
60	0.00271276516268443\\
61	0.00271394665440766\\
62	0.00238630217363459\\
63	0.0018840965738221\\
64	0.00134840980810499\\
65	0.000874593253390149\\
66	0.000508548145103344\\
67	0.000257971351253078\\
68	0.000107561775685078\\
69	3.21614893047939e-05\\
70	5.74420644477991e-06\\
71	6.36650771751457e-06\\
72	1.80693871067172e-05\\
73	3.08445937799162e-05\\
74	3.95892827150246e-05\\
75	4.26999855943078e-05\\
76	4.0707489801034e-05\\
77	3.51614921683674e-05\\
78	2.78398594763252e-05\\
79	2.02728513814532e-05\\
80	1.3526428497751e-05\\
81	8.17034144606765e-06\\
82	4.35715395638581e-06\\
83	1.95022491827901e-06\\
84	6.55869239502005e-07\\
85	1.32775205385904e-07\\
86	6.71292349485597e-08\\
87	2.13127866244278e-07\\
88	4.05268921171986e-07\\
89	5.51569778239891e-07\\
90	6.1673393583761e-07\\
91	6.02476767419535e-07\\
92	5.29772368196291e-07\\
93	4.25439230428148e-07\\
94	3.13657453426819e-07\\
95	2.11841357206088e-07\\
96	1.2972741927908e-07\\
97	7.04294077780165e-08\\
98	3.23859806194982e-08\\
99	1.14267944273383e-08\\
100	8.63525639882567e-10\\
};\label{figGMSIE2}
\end{groupplot}
\node[anchor=south east, draw = black, line width=0.4pt, fill=white, font=\footnotesize]  (legend) at ([shift={(-1.9cm,0.1cm)}]fig3 c1r1.south east) {\begin{tabular}{l l}
NAG & \ref*{figNag3} \\
GM-SIE\(^1\) & \ref*{figGMSIE12}\\
Shi-SIE & \ref*{figshiSIE2}
\end{tabular}};

\node[anchor=south east, draw = black, line width=0.4pt, fill=white, font=\footnotesize,scale=0.9]  (legend) at ([shift={(-0.1cm,2.5cm)}]fig3 c2r1.south east) {\begin{tabular}{l l}
NAG & \ref*{figNag4} \\
GM-SIE\(^1\) & \ref*{figGMSIE1}\\
GM-SIE\(^2\) & \ref*{figGMSIE2}
\end{tabular}};

%
\end{tikzpicture}%
